Synthesizing Physical Character-Scene Interactions

Movement is how people interact with and affect their environment. For realistic character animation, it is necessary to synthesize such interactions between virtual characters and their surroundings. Despite recent progress in character animation using machine learning, most systems focus on controlling an agent's movements in fairly simple and homogeneous environments, with limited interactions with other objects. Furthermore, many previous approaches that synthesize human-scene interactions require significant manual labeling of the training data. In contrast, we present a system that uses adversarial imitation learning and reinforcement learning to train physically-simulated characters that perform scene interaction tasks in a natural and life-like manner. Our method learns scene interaction behaviors from large unstructured motion datasets, without manual annotation of the motion data. These scene interactions are learned using an adversarial discriminator that evaluates the realism of a motion within the context of a scene. The key novelty involves conditioning both the discriminator and the policy networks on scene context. We demonstrate the effectiveness of our approach through three challenging scene interaction tasks: carrying, sitting, and lying down, which require coordination of a character's movements in relation to objects in the environment. Our policies learn to seamlessly transition between different behaviors like idling, walking, and sitting. By randomizing the properties of the objects and their placements during training, our method is able to generalize beyond the objects and scenarios depicted in the training dataset, producing natural character-scene interactions for a wide variety of object shapes and placements. The approach takes physics-based character motion generation a step closer to broad applicability.

==> FIG_autoencoder.tex <==
\begin{figure}[!h]
	\centering	
	\includegraphics[width=\linewidth]{figures/object_autoencoder.png}
	\caption{
	Autoencoder.
	}
	\label{fig:autoencoder}
\end{figure}


==> FIG_perturbations.tex <==
\begin{figure*}
	\centering	
	\includegraphics[width=\linewidth]{figures/projectiles.png}	
	\caption{
	Robustness to physical perturbations.
	}
	\label{fig:perturbations}
\end{figure*}

==> FIG_target_positions.tex <==
\begin{figure}
	\centering	
	\includegraphics[width=\linewidth]{example-image-a}	
	\caption{
	Target positions.
	}
	\label{fig:target_positions}
\end{figure}

==> FIG_visual_baselines.tex <==
\begin{figure}
	\centering	
	\includegraphics[width=\linewidth]{example-image-a}	
	\caption{
	Comparison with NSM~\cite{nsm_2019},SAMP~\cite{hassan_samp_2021}, and Chao \etal ~\cite{chao2019learning_to_sit}.
	}
	\label{fig:visual_baselines}
\end{figure}

==> TAB_compare_success_rate.tex <==
\begin{table}[]
\caption{Comparing success rate}
\begin{tabular}{|c|c|c|c|c|}
\hline
Method    & Sit & lie down & lift & carry \\ \hline
NSM~\cite{nsm_2019}       &     &    N/A     &      &     N/A  \\ \hline
SAMP~\cite{hassan_samp_2021}      &     &         &   N/A   &   N/A    \\ \hline
Chao \etal ~\cite{chao2019learning_to_sit}     &   $17\%$  &   N/A      &  N/A    &   N/A    \\ \hline
\modelname &   $90\%$  &         &      &  $98.9\%$     \\ \hline
\end{tabular}

\label{tab:compare_success_rate}
\end{table}

==> TAB_traj_compare.tex <==
\begin{table}[]
\caption{Trajectory Comparison}
\label{tab:traj_compare}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Task} & \textbf{Refrence Motion} & \textbf{Policy} \\ \hline
Sit           &                          &                 \\ \hline
Lie down      &                          &                 \\ \hline
Carry         &                          &                 \\ \hline
\end{tabular}
\end{table}
